Towards more patient friendly clinical notes through language models and ontologies

Clinical notes are an efficient way to record patient information but are notoriously hard to decipher for non-experts. Automatically simplifying medical text can empower patients with valuable information about their health, while saving clinicians time. We present a novel approach to automated simplification of medical text based on word frequencies and language modelling, grounded on medical ontologies enriched with layman terms. We release a new dataset of pairs of publicly available medical sentences and a version of them simplified by clinicians. Also, we define a novel text simplification metric and evaluation framework, which we use to conduct a large-scale human evaluation of our method against the state of the art. Our method based on a language model trained on medical forum data generates simpler sentences while preserving both grammar and the original meaning, surpassing the current state of the art.

==> algorithms/simplification.tex <==
 \begin{algorithm}[t]
     \begin{algorithmic}[1]
         \Statex \textbf{Input:} Clinician-written phrase/sentence $\textbf{sent}$.\vspace{5pt}

         \State $\con{ExpandedSent} := \con{abbreviationExp}(\textbf{sent})$	
         \State Let $n$ be term in $\textbf{sent}$
         \State Let $N$ be concept found in ont  $\textbf{O}$ containing term $n_{ont}=n$ and $m$ synonyms
         \Repeat {$\langle n_{ont1},..,n_{ontm}\rangle\in\con{synonyms}$}
            \State $\con{synScore} := \con{scoreSyn}(\textbf{sent}, \mathbf{n_{onti}})$
            \State $\con{bestSyn} := \con{argmax}(\textbf{synScore})$
            \State $\con{simpSent} := \con{subst}(\textbf{bestSyn, sent})$
         \Until {$convergence$}
         \State Replace $n$ in $\textbf{sent}$ with $n_{bestSyn}$
     \end{algorithmic}
     \caption{Simplification algorithm}
     \label{al:simple}
 \end{algorithm}


==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:acknowledgements}


==> tables/alpha.tex <==
\begin{table}[t]
    \centering
    \caption{Best\todo{Incorporate this table inside the caption of the alpha graph} Alpha according to SARI}
    \small
    \addtolength{\tabcolsep}{-1pt}
    \begin{tabular}{lccc}
        \hline
        \textbf{Model} & \textbf{Alpha} \\
        \hline
        Reddit-n-gram       &  0.70   \\
        \hline
        Reddit-GPT-1       &  0.90   \\
        \hline
        General-GPT-2       &  0.60  \\
        \hline
    \end{tabular}
    \label{tab:alpha}
\end{table}

==> tables/convergence.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Example of convergence}
%     \small
%     \addtolength{\tabcolsep}{-1pt}
%     \begin{tabular}{|p{1.3cm}|p{5.8cm}|}
%          \hline
%         \textbf{Iteration} & \textbf{Sentence} \\
%         \hline
%         Original    & hyperlipidemia with elevated triglycerides . \\
%         \hline
%         Iteration 1 & \textcolor{RoyalBlue}{elevated lipids in blood} \textcolor{RoyalBlue}{in addition to} \textcolor{RoyalBlue}{high} triglycerides .\\
%         \hline
%         Iteration 2 & \textcolor{RoyalBlue}{excessive fat} in \textcolor{RoyalBlue}{the} blood \textcolor{RoyalBlue}{with} high triglycerides .\\
%         \hline
%     \end{tabular}
%     \label{tab:convergence}
% \end{table}



==> tables/convergence_ablation.tex <==
\begin{table*}[h]
    \centering
    \caption{Convergence Ablation. Human judgement counts for sentence pairs from the test set for all models sentences. \textbf{S:} the generated was simpler; \textbf{F:} the original was simpler; \textbf{E:} both of equal complexity; \textbf{N:} cannot understand either; \textbf{SG:} simplification gain as defined in Equation \ref{eq:ratio}. Bold indicates best model.}

    \begin{tabular}{k|jjjj|j}
              \multicolumn{1}{s}{~} &
              \multicolumn{1}{s}{\textbf{S}}    & \multicolumn{1}{s}{\textbf{F}}    & \multicolumn{1}{s}{\textbf{E}}    & \multicolumn{1}{s}{\textbf{N}}    & \multicolumn{1}{s}{\textbf{SG}}    \\
        \hline
        \hline
        n-gram  (converged) & \textcolor{OliveGreen}{200} & \textcolor{BrickRed}{\textbf{146}} & 196 & \textbf{11}  & \textcolor{NavyBlue}{\textbf{0.031}}  \\
        n-gram (1st iteration) & \textcolor{OliveGreen}{\textbf{203}} & \textcolor{BrickRed}{159} & \textbf{174} & 17 & \textcolor{NavyBlue}{0.025}  \\
        \hline
        
        GPT-1  (converged) & \textcolor{OliveGreen}{263} & \textcolor{BrickRed}{\textbf{193}}  & 349 & \textbf{21}  & \textcolor{NavyBlue}{\textbf{0.040}} \\
        GPT-1  (1st iteration) & \textcolor{OliveGreen}{\textbf{285}} & \textcolor{BrickRed}{218}  & \textbf{294} & 29 & \textcolor{NavyBlue}{0.038} \\
        \hline
        
        
        GPT-2  (converged) & \textcolor{OliveGreen}{235} & \textcolor{BrickRed}{218} & \textbf{247} & \textbf{14} & \textcolor{NavyBlue}{0.010}\\
        GPT-2  (1st iteration) & \textcolor{OliveGreen}{\textbf{237}} & \textcolor{BrickRed}{\textbf{208}} & 285 & 19 & \textcolor{NavyBlue}{\textbf{0.016}}\\
    \end{tabular}
    \label{tab:convergence_ablation}
\end{table*}

==> tables/old/mainEvaluation.tex <==
\begin{table*}[htbp]
    \centering
    \small
        \begin{tabular}{lc|cccc}
            \hline
            \multicolumn{1}{l}{\textbf{Measure}}  &  
            \multicolumn{1}{l}{\textbf{Ref.}}  &
            \multicolumn{1}{l}{\textbf{ngram}}  &
            \multicolumn{1}{l}{\textbf{GPT1}}  &
            \multicolumn{1}{l}{\textbf{GPT2-G}}  &
            \multicolumn{1}{l}{\textbf{NMT}}  \\
            \hline
            1 – Simpler than orig. & \textcolor{OliveGreen}{\textbf{1730}} & \textcolor{OliveGreen}{\textbf{1452}} & \textcolor{OliveGreen}{1404} & \textcolor{OliveGreen}{1372} & \textcolor{OliveGreen}{587} \\
            (SimpleScore) & \textcolor{OliveGreen}{\textbf{\emph{\scriptsize{24.71\%}}}} & \textcolor{OliveGreen}{\textbf{\emph{\scriptsize{20.74\%}}}} & \textcolor{OliveGreen}{\emph{\scriptsize{20.06\%}}} & \textcolor{OliveGreen}{\emph{\scriptsize{19.60\%}}} & \textcolor{OliveGreen}{\emph{\scriptsize{8.39\%}}} \\

            2 – harder than orig. & \textcolor{BrickRed}{\textbf{273}} & \textcolor{BrickRed}{1004} & \textcolor{BrickRed}{\textbf{747}} & \textcolor{BrickRed}{1077} & \textcolor{BrickRed}{855} \\
            & \textcolor{BrickRed}{\textbf{\emph{\scriptsize{3.90\%}}}} & \textcolor{BrickRed}{\emph{\scriptsize{14.34\%}}} & \textcolor{BrickRed}{\textbf{\emph{\scriptsize{10.67\%}}}} & \textcolor{BrickRed}{\emph{\scriptsize{15.39\%}}} & \textcolor{BrickRed}{\emph{\scriptsize{12.21\%}}} \\

            3 – same level & 904 & 1732 & 1736 & 1661 & 1022 \\
            & \emph{\scriptsize{12.91\%}} & \emph{\scriptsize{24.74\%}} & \emph{\scriptsize{24.80\%}} & \emph{\scriptsize{23.73\%}} & \emph{\scriptsize{14.60\%}} \\
            
            4 – equally hard & 40 & 110 & 117 & 118 & 98 \\
            & \emph{\scriptsize{0.57\%}} & \emph{\scriptsize{1.57\%}} & \emph{\scriptsize{1.67\%}} & \emph{\scriptsize{1.69\%}} & \emph{\scriptsize{1.40\%}} \\
            \hline
            
            RatioScore & \textcolor{NavyBlue}{\textbf{0.208}} & \textcolor{NavyBlue}{0.064} & \textcolor{NavyBlue}{\textbf{0.093}} & \textcolor{NavyBlue}{0.042} & \textcolor{NavyBlue}{$-$0.038}\\

            \hline
            Unchanged & 4053 & 2702 & 2996 & 2772 & 4438 \\
            & \emph{\scriptsize{57.90\%}} & \emph{\scriptsize{38.60\%}} & \emph{\scriptsize{42.80\%}} & \emph{\scriptsize{39.60\%}} & \emph{\scriptsize{63.40\%}} \\


            \hline
        \end{tabular}
    \caption{Human evaluation of simplification models}
    \label{tab:main_eval}
\end{table*}

==> tables/old/significance.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{p{1.1cm} p{1.1cm} p{1.1cm} p{1.2cm} p{1.1cm}}
     & \textbf{\small{ngram}} & \textbf{\small{GPT1}} & \textbf{\small{GPT2-G}} & \textbf{\small{NMT}}\\ 
    \hline
    \small{Ref} & \small{0.000**} & \small{0.000**} & \small{0.000**} & \small{0.000**} \\
    \small{ngram} &  & \small{0.007**} & \small{0.111} & \small{0.000**} \\
    \small{GPT1} &  &  & \small{0.000**} & \small{0.000**} \\
    \small{GPT2-G} &  &  & & \small{0.000**} \\
    \hline
    \multicolumn{3}{l}{\textsuperscript{**}$p<0.01$, 
      \textsuperscript{*}$p<0.05$}
\end{tabular}
\caption{P-values obtained from Chi-squared significance test on answer contingency table.}
\label{tab:significance}
\end{table}

% \subsection{Significance testing}

% To test significance of our findings, we compute Chi-squared tests on the contingency table of answer counts. Table \ref{tab:significance} shows P-values computed on answer counts. Only the model pair n-gram and GPT2-G fails to show significantly different answer distributions under the 0.05 significance level. The Chi-squared test on nominal data assumes no relationship between subjects in each group. Given there are 7 annotation for each sentence pair, we repeated the significance test after assigning the most frequent category to each sentence pair. We excluded all sentences from evaluation that did not reach a majority label, i.e. the label being selected by at least 4 out of the 7 annotators, resulting in 1575 unique sentence pairs. The resulting contingency table and significance test results can be found in Appendix Tables \ref{tab:appendix_contigency} and \ref{tab:appendix_significance}. 
% %The SimpleScore, Simplification Gain as well as the significance tests reproduce the results found on the answer count level. 

% \input{tables/significance.tex}

==> tables/onto_example.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Example of concepts in the vocabulary, created by merging three ontologies  ((s) - Snomed, (c) - CHV, (h) - HPO) }
%     \small
%     \addtolength{\tabcolsep}{-1pt}
%     \begin{tabular}{p{4cm}rr}
%         \hline
%         \multicolumn{1}{l}{\textbf{Concept label}}  &   \multicolumn{1}{r}{\textbf{Alternative labels}} \\
%         \hline
%         Myocardial Infarction          &   infarction of heart  (s)  \\
%                             &  attack hearts (c)\\
%                             &  heart attack (h) \\
%         \hline
%         Headache       &  cephalodynia (s)   \\  
%                             & pain in head (c) \\ 
%                             & headaches (h) \\
%         \hline
%         Otalgia         &   pain in ear (s)  \\ 
%                             & earache (c) \\
%                             & ear pain (h) \\
%         \hline
%         %        \textbf{Total}      &   120\,606       &  2\,421     \\
%         %        \hline
%     \end{tabular}
%     \label{tab:vocabulary}
% \end{table}


==> tables/readability.tex <==
\begin{table}[t]
    \centering
    \caption{U.S. readability grade level for original, human and model simplified text. \textbf{SI:} SMOG Index ~\cite{smogreadability}; \textbf{FK:} Flesch--Kincaid Grade Level ~\cite{kincaid1975derivation}; \textbf{GF: } Gunnning Fog Index ~\cite{gunningfog}}
    
\begin{tabular}{k|jjj}
    \multicolumn{1}{s}{\textbf{~}} & \multicolumn{1}{s}{\textbf{SI}} & \multicolumn{1}{s}{\textbf{FK}} & \multicolumn{1}{s}{\textbf{GF}}  \\
    \hline
    \hline
    Original     & 10.9 & 8.8 & 7.22 \\ \hline
    Human   & 10.9  & 7.2  & 7.6 \\ \hline
    GPT-1    & \textbf{10.5} & \textbf{6.7} & \textbf{7.01} \\
    NTS     & 11.0 & 7.0 & 7.77 \\
    \hline
    \end{tabular}
    
    % FRE: Flesch Reading Ease (higher value indicates ease of reading) ~\cite{kincaid1975derivation} \\ 
    % CLI: Coleman-Liau Index ~\cite{Coleman1975ACR}, NDCR: New Dale-Chall Readability Score ~\cite{ndcr}, LW: Linsear Write ~\cite{linsearwrite}, 
    \label{tab:readibility_scores}
\end{table}

==> tables/significance_SG.tex <==
\begin{table}[h]
    \centering
        \caption{Results of approximate randomisation significance tests \cite{Efron1987} on simplification gain $SG$ scores presented in Table \ref{tab:human_eval}}
\begin{tabular}{k|jjjj}
              \multicolumn{1}{s}{~} &
              \multicolumn{1}{s}{\textbf{n-gram}}    & \multicolumn{1}{s}{\textbf{GPT-1}}    & \multicolumn{1}{s}{\textbf{GPT-2}}    & \multicolumn{1}{s}{\textbf{NTS}}    \\
        \hline
        \hline
        Human   & 0.000** & 0.000** & 0.000** & 0.000** \\ 
        \hline
        n-gram  & \multicolumn{1}{s}{\textbf{-}} & 0.000** & 0.025* & 0.000** \\
        GPT-1   & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & 0.000** & 0.000** \\
        GPT-2   & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & 0.000** \\
        \hline
        \multicolumn{2}{s}{\textsuperscript{**} $p<0.01$, 
      \textsuperscript{*} $p<0.05$}
    \end{tabular}
    \label{tab:significance_SG}
\end{table}


==> tables/significance_f1.tex <==
\begin{table}[h]
    \centering
        \caption{Results of approximate randomisation significance tests \cite{Efron1987} on F1--scores presented in Table \ref{tab:ref_metrics}.}
\begin{tabular}{k|jjjj}
              \multicolumn{1}{s}{~} &
              \multicolumn{1}{s}{\textbf{n-gram}}    & \multicolumn{1}{s}{\textbf{GPT-1}}    & \multicolumn{1}{s}{\textbf{GPT-2}}    & \multicolumn{1}{s}{\textbf{NTS}}    \\
        \hline
        \hline
        Human   & 0.000** & 0.000** & 0.000** & 0.000** \\ 
        \hline
        n-gram  & \multicolumn{1}{s}{\textbf{-}} & 0.970 & 0.091 & 0.000** \\
        GPT-1   & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & 0.252 & 0.000** \\
        GPT-2   & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & \multicolumn{1}{s}{\textbf{-}} & 0.000** \\
        \hline
        \multicolumn{2}{s}{\textsuperscript{**} $p<0.01$, 
      \textsuperscript{*} $p<0.05$}
    \end{tabular}
    \label{tab:significance_f1}
\end{table}
